Precision dispersive approaches versus unitarized Chiral Perturbation Theory for the lightest scalar resonances $\sigma/f_0(500)$ and $\kappa/K_0^*(700)$

For several decades, the $\sigma/f_0(500)$ and $\kappa/K_0^*(700)$ resonances have been subject to long-standing debate. Both their existence and properties were controversial until very recently. In this tutorial review we compare model-independent dispersive and analytic techniques versus unitarized Chiral Perturbation Theory, when applied to the lightest scalar mesons $\sigma/f_0(500)$ and $\kappa/K_0^*(700)$. Generically, the former have settled the long-standing controversy about the existence of these states, providing a precise determination of their parameters, whereas unitarization of chiral effective theories allows us to understand their nature, spectroscopic classification and dependence on QCD parameters. Here we review in a pedagogical way their uses, advantages and caveats.

==> sections/anastructure.tex <==
In the right panel of Fig.~\ref{fig:mNmmN} we have depicted the
$M_1(p_1)M_2(p_2)\rightarrow M_1(p_3)M_2(p_4)$ scattering process, where $p_i$ are the meson four-momenta and in our case $M_1M_2=\pi\pi$ or $\pi K$. The corresponding amplitude is denoted as $F(s,t,u)$, where $s,t,u$ are the usual Mandelstam variables explained in the plot, with 
$ u=\sum_i m_i^2-s-t$. It is more convenient to use amplitudes with a given isospin, which we assume conserved, and since $u$ is redundant as a variable, to write the amplitudes as $F^I(s,t)$. 

We will be mostly interested in partial-waves of definite angular momentum and isospin since in that way we can identify the spin and quantum numbers of the resonances observed on each partial wave. 
These partial waves are obtained from by the usual projection:
$$F^I(s,t)=16\pi K\sum_{\ell=0}^{\infty}(2\ell+1)P_\ell(z_s)F_{ij}(s),\; F_{ij}(s)=\frac{1}{32\pi K}\int_{-1}^{1} dz_s P_\ell(z_s) F^I(s, t(z_s)),$$
where $P_\ell$ are the Legendre polynomials and $z_s$ is the scattering angle in the $s$ channel. Note that $K=1,2$ for $K\pi$ and $\pi\pi$, respectively, because, form the point of view of hadron interactions, pions are identical particles in the isospin limit that we are considering here. 

Let us also recall that it is more convenient to recast partial waves in terms of the phase shift $\delta_\ell^I$ and elasticity $\eta_\ell^I$\footnote{In the literature these are also written as $\delta_{I\ell},\delta^{(I)}_\ell$ and
 $\eta_{I\ell},\eta^{(I)}_\ell$ as we will see in several figures of this tutorial review} as follows:
\begin{equation}
f_\ell^I(s)=\frac{\eta_\ell^I(s) e^{i2\delta_\ell^I(s)}-1}{2i\sigma(s)},\quad \sigma(s)=\frac{2q(s)}{\sqrt{s}}
\label{eq:phasespace}
,\end{equation}
where $q$ is the CM momentum of the scattering particles. In the elastic regime $\eta_\ell^I=1$ and we can write:
\begin{equation}
f_\ell^I(s)=\frac{ e^{i\delta_\ell^I(s)}\sin \delta_\ell^I(s)}{\sigma(s)}.
\label{eq:felastic}
\end{equation}

In order to understand the relevance of analyticity for the determination of the $\sig$ and $\kap$ as poles in the complex plane, we first have to describe the analytic structure of meson-meson scattering partial waves (see \cite{Pelaez:2015qba,Pelaez:2020gnd} for a pedagogical detailed introduction and review). Thus, in the upper and lower panels of Fig.~\ref{fig:anstruc} we show the analytic structure of  $\pi\pi$ and $K \pi$ scattering partial waves, respectively.  Note that we are showing the $s$-plane, which is the Lorentz invariant variable in which partial-waves are analytic in the whole complex plane, except for several cuts. Some features are common to the two cases: 1) partial-waves satisfy Schwartz symmetry, $f(s^*)=f(s)^*$; 2) the right cut on the real axis, also known as physical or unitarity cut, extending from threshold to $+\infty$, which can overlap with other cuts when additional states become available. The physical value of the partial wave is evaluated precisely over this cut as $f(s)=f(s+i\epsilon)$ with $0<\epsilon\rightarrow0$; 3) The presence of Adler zeros on the real axis below threshold, which are dynamical features required by the spontaneous chiral symmetry breaking, due to the pseudo-NGB nature of pions and kaons; 4) A left cut coming from $-\infty$ and extending to the square of the mass difference between the incoming mesons. This cut is due to the presence of physical cuts in crossed channels, as seen from the $s$-channel. Finally, there is a circular cut centered at $s=0$  whose radius is the difference of the squared masses of the incoming mesons (which collapses to the origin for $\pi\pi$ scattering). Poles in the real axis could exist below threshold, signaling the presence of bound states. But they do not exist for $\pi\pi$ or $K\pi$ scattering, and causality guarantees that no other singularities exist in the so called first Riemman sheet, where the CM momentum as a complex variable has a positive imaginary part, of partial waves.

However, when promoting the momentum to a complex variable, it can also have a negative imaginary part, and that defines a second Riemann sheet, accessible from the first by crossing continuously the first sheet. Actually, the number of sheets doubles every time a new accessible state, with its own associated CM  momentum,  becomes available. In these ``unphysical sheets" other singularities can appear, like pairs of conjugates poles.
When these poles are very close to the real axis and isolated from other singular structures, from the real axis they are seen as ``peaks" in the squared partial wave and the cross section. This is the case of typical resonances like the $\rho(770)$ or $K^*(892)$, whose positions $\sqrt{s_{pole}}=M_R-i\Gamma_R/2$ we illustrate in the figure. In such cases, the phase shift in the real axis has a shape as that shown in the left panel of Fig.~\ref{fig:dataraw}, reaching $90^\degree$ at $s=M_R^2$, and the familiar Breit-Wigner description is a fairly good approximation. In these cases Note that, out of their associated conjugate pair of poles, we are only showing the one in the lower half plane, which is the one that most affects the partial wave in the real axis. In contrast, we are also showing the $f_0(980)$ pole position, but it is so close to the opening of the $K\bar K$ threshold that a naive Breit-Wigner shape is not valid. Actually, it produces a dip in the cross section, not a peak, because, as seen in the left panel of Fig.~\ref{fig:dataraw}, the phase shift around 980 MeV is not $90^\degree$ but relatively closer to $180^0$.

The situation is even more complicated for the $\sig$ and $\kap$ poles, which, as seen in Fig.~\ref{fig:anstruc}
lie deep in the second Riemann sheet of the complex plane. Moreover, they lie as close to the real axis in their nominal mass region as they do to other analytic features like the threshold or the left and circular cuts. An analytic continuation deep in the complex plane is a delicate extrapolation from the real axis, but in these cases, it is even hindered by the presence of these other analytic structures, for which we need to have some reasonable control if we are to claim a precise determination of these pole parameters. Even the Adler zero, despite lying in the first Riemann sheet, is rather close to the pole, and its absence can deform the whole amplitude.

As an example, we have recently shown that an inconsistent treatment of the unphysical cuts can yield move the pole-width  of the $\kap$ by 200 MeV, {\it even if using the same fit to data in the \kap region}. These are the two ``UFD" results in Fig.~\ref{fig:kappapoles}. 

Therefore, to have a precise determination of the pole we need both reliable data and a sound analytic formalism. Both goals can be achieved with dispersion relations.


\begin{figure}
\begin{center}
% Use the relevant command for your figure-insertion program
% to insert the figure file.
% For example, with the option graphics use
\resizebox{1.\columnwidth}{!}{%
  \includegraphics{Anstruc-pw} }
\caption{Analytic structure of meson-meson scattering partial waves in the complex-$s$ plane. They always have a right cut, also called physical or unitarity cut, starting at the first two-body threshold and extending to $+\infty$, as well as a left cut extending from $s=0$ to $-\infty$. For the case of different mass mesons there is also a circular cut and the left cut extends further from $s=0$ to the square of their mass difference. Top: For  $\pi\pi$ scattering  we illustrate the position of the known $\sig$, $\rho(770)$ and $f_0(980)$ resonance poles, in the second Riemann sheet. Note that the \sig pole is similarly close to the resonance nominal mass than to threshold, the left cut or the Adler zero required by chiral.
 symmetry (which lies on the first sheet). Bottom: For $\pi K$ scattering we show the $K^*(892)$ and \kap poles in the second Riemann sheet
 Note that the latter is roughly as close to the real axis around the resonance nominal mass than it is to other analytic features. The bottom figure is taken from  \cite{Pelaez:2020gnd}.}
\label{fig:anstruc}       % Give a unique label
\end{center}
\end{figure}
